Efficient Profile Maximum Likelihood for Universal Symmetric Property Estimation

Estimating symmetric properties of a distribution, e.g. support size, coverage, entropy, distance to uniformity, are among the most fundamental problems in algorithmic statistics. While each of these properties have been studied extensively and separate optimal estimators are known for each, in striking recent work, Acharya et al. 2016 showed that there is a single estimator that is competitive for all symmetric properties. This work proved that computing the distribution that approximately maximizes \emph{profile likelihood (PML)}, i.e. the probability of observed frequency of frequencies, and returning the value of the property on this distribution is sample competitive with respect to a broad class of estimators of symmetric properties. Further, they showed that even computing an approximation of the PML suffices to achieve such a universal plug-in estimator. Unfortunately, prior to this work there was no known polynomial time algorithm to compute an approximate PML and it was open to obtain a polynomial time universal plug-in estimator through the use of approximate PML. In this paper we provide a algorithm (in number of samples) that, given $n$ samples from a distribution, computes an approximate PML distribution up to a multiplicative error of $\exp(n^{2/3} \mathrm{poly} \log(n))$ in time nearly linear in $n$. Generalizing work of Acharya et al. 2016 on the utility of approximate PML we show that our algorithm provides a nearly linear time universal plug-in estimator for all symmetric functions up to accuracy $\epsilon = \Omega(n^{-0.166})$. Further, we show how to extend our work to provide efficient polynomial-time algorithms for computing a $d$-dimensional generalization of PML (for constant $d$) that allows for universal plug-in estimation of symmetric relationships between distributions.

==> appoverview.tex <==
\section{Overview of appendix}
Here we provide the overview of appendix. First, we provide all the proofs for the one dimensional PML. Specifically in \Cref{sec:prelims}, we redefine all the old (defined in \Cref{sec:prelimsmain}) and introduce some more new definitions. In \Cref{sec:structure}, we provide the detailed proof of \Cref{thm:approxpml} by restating all the lemmas from \Cref{sec:structuremain} in the main paper. In \Cref{app:universal}, we provide the proof for \Cref{theoremADOSuniversal} that relates approximate PML distribution to universal plug-in estimator. In sections \ref{app:minprob} and \ref{app:structure}, we provide the remaining proofs from \Cref{sec:structure}. In \Cref{app:cuttingplane}, we provide an algorithm to solve the convex relaxation of SDPML (defined in \Cref{sec:structuremain} and redefined again in \Cref{sec:structure}). 

In the remaining part of the appendix (sections \ref{app:multipmlstart} and \ref{sec:multpmlremain}) we provide proofs for the higher dimensional PML. Proofs for the higher dimensional PML follow similar structure as the one dimensional PML but need more general arguments. We recommend readers to first go through the one dimensional case first as it captures all the main ideas.
